Experiments with Encoding Structured Data for Neural Networks

The project's aim is to create an AI agent capable of selecting good actions in a game-playing domain called Battlespace. Sequential domains like Battlespace are important testbeds for planning problems, as such, the Department of Defense uses such domains for wargaming exercises. The agents we developed combine Monte Carlo Tree Search (MCTS) and Deep Q-Network (DQN) techniques in an effort to navigate the game environment, avoid obstacles, interact with adversaries, and capture the flag. This paper will focus on the encoding techniques we explored to present complex structured data stored in a Python class, a necessary precursor to an agent.

==> 0-TODO_LIST.tex <==
%TC:ignore
\noindent
\pagenumbering{roman}

Version: \DTMnow{} $\approx$
9661
words \hfill \reportOnFIXME

{\footnotesize
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
\tableofcontents
%\listoftables
%\listoffigures
}

\textbf{\LARGE{TODO\_LIST}}
\begin{enumerate}

\item There are a few peculiarities about the organization of this.
First, ensure that the MAIN .tex and the .bib are ON THE TOP LEVEL AND NAMED THE SAME THING. 
Failure to do so will make submission to arXiv via automatically download/uploading more complicated. 
The rest of this file is just some example formattings from old files.

\end{enumerate}


\textbf{\LARGE{TODO-LIST}}
\begin{enumerate}

\item do the thing

\end{enumerate}

\newpage
\setcounter{page}{1}
\pagenumbering{arabic}
%TC:endignore
